Understanding the Potential of FPGA-Based Spatial Acceleration for Large Language Model Inference

Recent advancements in large language models (LLMs) boasting billions of parameters have generated a significant demand for efficient deployment in inference workloads. The majority of existing approaches rely on temporal architectures that reuse hardware units for different network layers and operators. However, these methods often encounter challenges in achieving low latency due to considerable memory access overhead. This paper investigates the feasibility and potential of model-specific spatial acceleration for LLM inference on FPGAs. Our approach involves the specialization of distinct hardware units for specific operators or layers, facilitating direct communication between them through a dataflow architecture while minimizing off-chip memory accesses. We introduce a comprehensive analytical model for estimating the performance of a spatial LLM accelerator, taking into account the on-chip compute and memory resources available on an FPGA. Through our analysis, we can determine the scenarios in which FPGA-based spatial acceleration can outperform its GPU-based counterpart. To enable more productive implementations of an LLM model on FPGAs, we further provide a library of high-level synthesis (HLS) kernels that are composable and reusable. This library will be made available as open-source. To validate the effectiveness of both our analytical model and HLS library, we have implemented BERT and GPT2 on an AMD Alveo U280 FPGA device. Experimental results demonstrate our approach can achieve up to 13.4x speedup when compared to previous FPGA-based accelerators for the BERT model. For GPT generative inference, we attain a 2.2x speedup compared to DFX, an FPGA overlay, in the prefill stage, while achieving a 1.9x speedup and a 5.7x improvement in energy efficiency compared to the NVIDIA A100 GPU in the decode stage.

==> fig-tex/3d-parallelism.tex <==
\begin{figure}[!htbp]
    \centering
       
    \begin{subfigure}[b]{0.47\linewidth}
        \includegraphics[width=\linewidth]{figs/Data Parallelism.pdf}
        \caption{Data parallelism.}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\linewidth]{figs/Tensor Parallelism.pdf}
        \caption{Tensor parallelism}    
    \end{subfigure}
    
    \begin{subfigure}[t]{0.71\linewidth}
        \includegraphics[width=\linewidth]{figs/Pipeline Parallelism.pdf}    
        \caption{Pipeline parallelism}
    \end{subfigure}

    \caption{Parallelism schemes.}
    \label{fig:3d-parallelism}
\end{figure}


==> figs/models.tex <==
\begin{table}[!htbp]
\caption{Models used in the single-node experiments. \# of params shows the model size. MLM $=$ Mask language modeling. CLM $=$ Causal language modeling. Seq2Seq $=$ Sequence-to-Sequence modeling. IC $=$ Image Classification.}
\label{tab:models}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccc}\Xhline{2\arrayrulewidth}
\textbf{Model} & \textbf{Task} & \begin{tabular}{c}\textbf{\# of params}\\\textbf{(Billion)}\end{tabular} & \begin{tabular}{c}\textbf{Seq Length} /\\\textbf{Image Size}\end{tabular} & \textbf{Precision}\\\hline
BERT~\cite{devlin2018bert} & MLM & 0.96 & 512 & FP16 \\\hline
RoBERTa~\cite{liu2019roberta} & MLM & 1.3 & 512 & FP16\\\hline
GPT~\cite{radford2019gpt2} & CLM & 2.86 & 1024 & FP16\\\hline
OPT~\cite{zhang2022opt} & CLM & 2.69 & 1024 & FP16\\\hline
T5~\cite{2020t5} & Seq2Seq & 2.85 & 1024, 512 & FP16\\\hline
WideResNet~\cite{zagoruyko2016wide} & IC & 2.4 & 3$\times$224$\times$224 & FP32\\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\end{table}

\begin{comment}
\begin{table}[!htbp]
\caption{Models used in the experiments. \# of params shows the model size used in single-node experiments. MLM $=$ Mask language modeling. CLM $=$ Causal language modeling. Seq2Seq $=$ Sequence-to-Sequence modeling. IC $=$ Image Classification.}
\label{tab:models}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccc}\Xhline{2\arrayrulewidth}
\textbf{Model} & \textbf{Task} & \begin{tabular}{c}\textbf{\# of params}\\\textbf{(Million)}\end{tabular} & \begin{tabular}{c}\textbf{Seq Length} /\\\textbf{Image Size}\end{tabular} & \textbf{Precision}\\\hline
BERT~\cite{devlin2018bert} & MLM & 335 & 512 & FP16 \\\hline
RoBERTa~\cite{liu2019roberta} & MLM & 355 & 512 & FP16\\\hline
ALBERT~\cite{lan2020albert} & MLM & 177 & 512 & FP16\\\hline
GPT~\cite{radford2019gpt2} & CLM & 1300 & 1024 & FP16\\\hline
OPT~\cite{zhang2022opt} & CLM & 350 & 1024 & FP16\\\hline
T5~\cite{2020t5} & Seq2Seq & 770 & 1024, 512 & FP16\\\hline
WideResNet~\cite{zagoruyko2016wide} & IC & 250 & 3$\times$224$\times$224 & FP32\\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\end{table}
\end{comment}
